Beyond BatchNorm: Towards a Unified Understanding of Normalization in Deep Learning

Inspired by BatchNorm, there has been an explosion of normalization layers in deep learning. Recent works have identified a multitude of beneficial properties in BatchNorm to explain its success. However, given the pursuit of alternative normalization layers, these properties need to be generalized so that any given layer's success/failure can be accurately predicted. In this work, we take a first step towards this goal by extending known properties of BatchNorm in randomly initialized deep neural networks (DNNs) to several recently proposed normalization layers. Our primary findings follow: (i) similar to BatchNorm, activations-based normalization layers can prevent exponential growth of activations in ResNets, but parametric techniques require explicit remedies; (ii) use of GroupNorm can ensure an informative forward propagation, with different samples being assigned dissimilar activations, but increasing group size results in increasingly indistinguishable activations for different samples, explaining slow convergence speed in models with LayerNorm; and (iii) small group sizes result in large gradient norm in earlier layers, hence explaining training instability issues in Instance Normalization and illustrating a speed-stability tradeoff in GroupNorm. Overall, our analysis reveals a unified set of mechanisms that underpin the success of normalization methods in deep learning, providing us with a compass to systematically explore the vast design space of DNN normalization layers.

==> backup.tex <==
\section{Introduction}
Normalization layers are often necessary to effectively train deep neural networks (DNNs) with several layers (\cite{BN, LN, IN, GN}). Arguably, the most popular of these layers is BatchNorm (\cite{BN}), whose success can be attributed to its several benefits, such as, ability to train deeper models (\cite{rank_collapse}), support for large learning rates per iteration (\cite{fim, understanding_bn}), auto-tuning of learning rates throughout training (\cite{arora}), implicit regularization (\cite{pluo}), reduced dependence on initialization (\cite{skipinit, dispense_norm, fixup}), and improved loss landscape (\cite{santurkar, GC}). However, depending on the application scenario, BatchNorm's benefits can be limited or even harmful. For example, BatchNorm is known to struggle in settings where small batch-sizes have to be used (\cite{GN, batch_rn, transnorm}); its activation-centering operation results in decorrelated activations, which can lead to training instability due to gradient explosion (\cite{mft_bn}); in adversarial training, it can hamper performance on both clean and adversarial examples (\cite{adv_bn, advprop}); and in meta-learning, it can implicitly lead to transductive training (\cite{tasknorm}). 

To address these shortcomings, several recent works have tried to replace BatchNorm by designing normalization layers capable of either emulating some of its desirable \emph{benefits}, while avoiding some of its \emph{limitations}. For example, Brock et al.~\cite{nfnets_1, nfnets_2}) propose to replace BatchNorm with Scaled Weight Standardization~\cite{WS, cwn}, which matches the forward signal propagation behavior of BatchNorm in Residual networks. Singh and Krishnan~\cite{FRN} argue the mean operation of BatchNorm is unnecessary and propose Filter Response Normalization, which allows training of complex applications without batch dependence. Xie et al.~\cite{advprop} propose to use separate BatchNorm layers for adversarial examples to avoid learning of noisy statistics from perturbed examples during adversarial training. Overall, these past works (see \autoref{sec:related} for more examples) have successfully achieved their targeted properties, but it remains unclear if focusing on certain, specific attributes of BatchNorm can result in a general module capable of serving as its replacement.

\begin{table}[]
\centering
\caption{\label{tab:props}%
Benefits and limitations of BatchNorm and which operations gives rise to them in what mode (backward/forward).}
\begin{tabular}{@{}c|c|c@{}}
\toprule
Backward Mode          & Property                           & (+) Benefit/(-) Limitation                       \\ \midrule
Mean-centering         & Outlier eigenvalue removal         & (+) Allows large LR                      \\
                       & Reduced gradient confusion         & (+) Faster training                      \\
Variance Normalization & Scale-invariance                   & (+) Auto rate-tuning                     \\
                       & Avoids rank collapse               & (+) Training of deep models              \\  \toprule
Forward Mode           & Property                           & Benefit/Limitation                       \\\midrule
Mean-centering         & Decorrelated activations           & (-) Gradient explosion                   \\
                       & Train/Test inconsistency           & (-) Performance loss in Non-IID Settings \\
Variance Normalization & Biases residual blocks to identity & (+) Avoid variance explosion             \\
                       & Train/Test inconsistency           & (-) Performance loss in Non-IID Settings \\ \bottomrule
\end{tabular}
\end{table}

Our work is an attempt to understand the benefits and limitations of BatchNorm in a unified manner. Specifically, we ascertain which BatchNorm operation (mean-centering or variance normalization) gives rise to which of its properties (see \autoref{tab:props}). Interestingly, we find most benefits of BatchNorm are a consequence of how its operations transform gradients during backward propagation: training completely fails if these transformations are removed. We further show most limitations of BatchNorm arise from its forward propagation behavior. For example, due to the mean-centering operation, activations at initialization become highly decorrelated, resulting in gradient explosion~\cite{mft_bn}. This isolation of operation-property relationships also allows us to demonstrate several drawbacks in proposed replacements of BatchNorm in prior work. For example, since forward propagation does not explain BatchNorm's benefits, using Scaled Weight Standardization~\cite{WS, cwn} to match BatchNorm's forward propagation characteristics~\cite{nfnets_1,nfnets_2} is unlikely to result in a robust replacement. Indeed, we find on non-residual CNNs, Scaled Weight Standardization suffers from high performance loss. 

Based upon our analysis, we propose a unified optimization framework for training DNNs, called BNTrain, which is capable of retaining the BatchNorm's benefits, while avoiding its limitations. Specifically, we use our ascertained operation-property relationships and design backward/forward propagation operations that can inherit BatchNorm's benefits, but do not suffer from its limitations. For example, by inheriting BatchNorm's auto rate-tuning, our framework has convergence guarantees to critical points for training with SGD. We show the robustness of our framework by training networks without normalization layers in several practical scenarios: in image classification, we see ...; in object detection, we see ...; in adversarial training, we see ...; in meta-learning, we see ...; in GAN-training, we see ...; in contrastive learning, we see ...; in continual learning, we see ...; in federated learning, we see ....




Through our analysis, we identify following benefits and limitations of a family of normalization methods in deep learning.

\begin{itemize}
    \item[\textbf{Sec. \ref{sec:lagrangian}.}] \textbf{Stabilization of gradient norms at initialization.}
    %
    \item[\textbf{Sec. \ref{sec:kinetic_asymmetry}.}] \textbf{Avoiding rank-collapse at initialization.} 
    %
    \item[\textbf{Sec. \ref{sec:noether_bregman}.}] \textbf{Avoiding exploding and vanishing gradient at initialization.} 
    %
    \item[\textbf{Sec. \ref{sec:scale_dynamics}.}] \textbf{Auto-tuning of effective learning rates.} 
    %
\end{itemize}


==> backup_discussions.tex <==

Background:
Science: Understanding BatchNorm


Engineering: Replacing BatchNorm with the norm zoo


Where we stand?:
Harnessing the understanding of BatchNorm to "..." norm zoo.

Issue: Norm zoo is only evaluated in terms of the final accuracy when they were introduced. 
Q: Do they inherit other properties of the BatchNorm (see below)?
Why care?: As a practitioner, if we have to select which normalization method is suitable for each application scenarios, we also want to know 
Our answer: 
Which 
Evo-norm S0





Properties:
- speed of convergence:
- rank collapse: ability of the deep representations to discriminate distinct input data
- better trainability with resnets
- scale invariance and auto-tuning of learning rates
- support for large learning rate per iteration: Hessian




Performance:
Final test accuracy


Contributions:
- There is the norm zoo. Some of them are successful in some applications, but others are not. We didn't have any theoretical grounding to understand why.
- We identify essential theoretical grounding by looking through the literature of understanding batchnorm, and demonstrate that we can now predict the success and failure modes of norm zoo.

1. BatchNorm is great, you can't train deepnets without it. 2. But, it has limitations in practically important settings due to its dependence of data statistics. 3. A lot of modifications of BatchNorm have been proposed to eliminate the limitations, while only inheriting the benefits. 4. 


- Through analysis of normalization methods beyond batch norm demonstrating benefits and limitations in 



The success of BatchNorm can be attributed to its ability to enable training of deeper models with minimal hyperparameter tuning and faster convergence. However, depending on the application scenario, BatchNorm's benefits can be limited or even harmful. For example, BatchNorm is known to struggle in applications with non-IID data distributions (e.g., federated learning). Recent works have proposed several normalization layers to address such scenarios; however, despite their empirical success, there is currently limited understanding of why these methods avoid BatchNorm's limitations or exactly what are the sources of BatchNorm's limitations. To answer this question, we conduct a thorough analysis of signal propagation abilities of 10 recently proposed normalization layers. 



Inspired by the success of BatchNorm, there has been an explosion of normalization methods in deep learning. While such methods often outperform BatchNorm in specific, benchmark settings, there is limited work evaluating the sources of their effectiveness. Further, while BatchNorm boasts a multitude of beneficial mechanisms, it currently remains unclear which normalization methods inherit which mechanisms and in what settings. Contributing to a growing body of work on design of normalization layers, we ask: Are there universal mechanisms behind the success of normalization techniques in deep learning? Can the lack of these mechanisms explain failure modes of a normalization method? To this end, we conduct a unified analysis of stability of forward and backward propagation in 10 recently proposed normalization layers. Relating these abilities with the performance of a normalization layer in different settings (large/small batch-size and large/small learning rate), we show the success of a normalization layer can be boiled down to existence of three essential properties: (a) capability to retain discriminative activation patterns in deep layers, (b) stability of gradient propagation across layers (i.e., neither exploding nor vanishing), and (c) robustness to scale of initial learning rate. 




While several recent work contribute to building a better understanding of BatchNorm, there are limited works analyzing which general mechanisms render a normalization layer successful?


address two question in this work: (i) Which properties of BatchNorm can be attributed to which of its operations? and (ii) Which BatchNorm properties are more useful for a replacement method to inherit? Ascertaining the existence of known properties of BatchNorm in recently proposed normalization layers and relating them to a layer's performance helps us determine which properties a replacement technique should try to inherit. 



Normalization layers are often necessary to effectively train deep neural networks (DNNs) with several layers. Arguably, the most popular of these layers is BatchNorm, whose success can be attributed to its several benefits, such as, ability to train deeper models, support for large learning rates per iteration, auto-tuning of learning rates throughout training, implicit regularization, reduced dependence on initialization, and improved loss landscape. However, depending on the application scenario, BatchNorm's benefits can be limited or even harmful. For example, BatchNorm is known to struggle in applications with non-IID data distributions (e.g., federated learning); it can result in increased vulnerability to adversarial examples; and in meta-learning, it can implicitly lead to transductive training. 








\textbf{Main contributions:}
\begin{enumerate}
    \item We demonstrate that each of the existing normalization methods has its own failure mode in different application scenarios.
    %
    \item To better understand which normalization methods work, when, and why
\end{enumerate}















\section{\red{Writing strategy}}
Figure 1 Main idea: Different properties hold and not hold well for different normalization methods; BatchNorm works well for most (not all). Start --> End: BN works well to not works well. Only accuracy plots: Different batch sizes and learning rates. 


\textbf{Q. What is the main issue that we are addressing?}\\
The existing literature mostly explore individual points in a vast space spanned by (i) normalization methods, (ii) mechanisms, (iii) application.
%
However, 



We combine ablation, correlation


\textbf{Who will benefit from this paper in what way?}\\
1. For a given application, which normalization should be used? What are the expected benefits and limitations?\\
2. When a normalization method is not working, what might be the reason? What should we plot to debug it? (rank-collapse? gradient explosion?)\\
3. For researchers designing new normalization methods, what are the existing challenges and bottlenecks?





\textbf{Approach}\\
In this paper, we intentionally focus on scientific approach, i.e., the aim of this paper is not to sell an algorithm, rather to test hypotheses.
%
One of the main issue in the existing literature is that scientific and engineering efforts are mixed up and people are faking to make it...


\textbf{Hypothesis 1. }















\section{Building blocks of batch normalization}
\label{section:building_blocks}

\textbf{Outline:}\\
1. Is it about forward prop or backward prop? Backward-prop (attack the motivation of NFNets, data-whitening arguments in understanding BN papers).\\
2. In backward prop, is mean-centering more important or variance normalization? mean-centering (attack the motivation of FRN).\\
3. If mean-centering is so important, then what is it doing: Controlling scale of activations and gradients. Can this be done in some other way? Yes, for example by using bounded activations (FRN, EvoNorm) or weight-centering. Are these solutions general? No, cannot support large learning rates.\\
4. What is variance normalization doing? Allowing larger LRs. Most recently proposed layers seem incapable of supporting large learning rates. Why? Huge gradient norms at initialization, thus demanding smaller learning rates.


\section{Benefits of batch normalization}
\label{section:benefits}

lecture note by Roger Grosse \cite{grosse2021nntd}

\textbf{Preventing internal covariate shift (ICS).}


\textbf{Preventing dead or saturated neurons.}
Gradient and activation correlation experiments (see Is BatchNorm unique and Shattered Gradients)

\textbf{Faster training.}\\
Generally, proposed replacements in past work don't show convergence plots. 

\textbf{Auto tuning of learning rates.}\\
Doesn't seem to hold for recently proposed layers.

\textbf{Smoothing of loss landscape.}\\
Generally true for all, but may be better to calculate exactly which layer has a smaller lipschitz constant.

\textbf{Stochastic regularization by batch sampling.}\\
I don't think this is actually a benefit, but just an intuitive argument. In fact, it may be hurting model performance.

\textbf{FC layer regularization.}\\
Won't hold for all normalization layers.


\section{Limitations of batch normalization}
\label{section:limitations}
Most limitations arise due to batch dependence, which results in inconsistent train/test behavior. We will compare replacement layers for:

\textbf{Continual learning.}



\textbf{Meta-learning or Transfer learning.}



\textbf{Adversarial training}


\textbf{Contrastive learning}


\textbf{Federated learning}


\textbf{Detection/Segmentation}


\section{How to Design Replacements of BatchNorm}
\label{section:replacements}
1. Activation controlling operations (centering; bounded activations (may lead to saturated gradients, though); maybe better can be designed)
2. Normalization operations (support scale invariance; avoid rank collapse; no batch-dependence, ideally)
3. Initialization (current ones work well with BatchNorm, but may not work for other layers) 


\section{Conclusion}








\clearpage
\textbf{Description:}\\
Fwd prop is a limited perspective on BN and other methods: Extensive ablations [Done]

\textbf{Training stability and other benefits may be at odds:}\\
Benefits of batch dependence: higher learning rate (scale invariance -> sparsity); control of activations (training stability); smoothness of landscapes; Contrastive learning.

\textbf{Limitations of batch dependence:}\\
Continual learning / meta-learning (smooth landscapes vs. batch statistics trade-off), Adversarial training.

\textbf{Applications beyond classification (Do recently proposed layers translate to other applications?):}\\
Detection; Segmentation; Contrastive Learning (Pos and Neg, both types of frameworks).

\textbf{Prescription:}\\
Think of BatchNorm as an optimizer: Include the backprop step into the optimization process somehow. 

\textbf{End Goal:}\\ 
Table of Properties for different layers: What recently proposed variant shares the properties that BatchNorm has (relate that with applications to show when it is useful).
Properties vs. Applications--Which property is valuable in which applications (clarifying the role of different property is valuable for which specific application).



\clearpage
\section{Q1. What are the benefits of batch normalization?}

based on lecture note by Roger Grosse \cite{grosse2021nntd}

\textbf{Solve the ill-conditioning effects of ICS (internal covariance shift)}

\textbf{Prevent dead or saturated units}

\textbf{Maintain stability at higher learning rates}

\textbf{A regularization effect resulting from the normalizer being stochastic depending on the minibatch}





\clearpage
\section{Introduction}
Batch normalization is...
%
Our main contributions are:
\begin{compactenum}
    \item We study ... (Sec. \ref{section:layer-collapse}).
    %
    \item We demonstrate ... (Sec. \ref{section:conservation}).
    %
    \item We show that ... (Sec. \ref{section:conservation}).
    %
    \item We hypothesize that ... (Sec. \ref{sec:itertaive-magnitude-pruning}).
    \item We prove that ... (Sec. \ref{sec:algorithm}).
    %
    \item  We introduce ... (Sec. \ref{section:experiments}).
\end{compactenum}



==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The results are distributed throughout the paper and closely follow the abstract's narrative.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, wherever applicable. We note our focus was analysis of an existing method, not proposal of a new method.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{Theoretical work, primarily.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \autoref{sec:stable_fwd}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See \autoref{sec:stable_fwd}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplementary.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See supplementary}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All results are averaged over 3 seeds}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See supplementary}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See supplementary}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
